Rapid and High-Fidelity Subsurface Exploration with Multiple Aerial Robots

This paper develops a communication-efficient distributed mapping approach for rapid exploration of a cave by a multi-robot team. Subsurface planetary exploration is an unsolved problem challenged by communication, power, and compute constraints. Prior works have addressed the problems of rapid exploration and leveraging multiple systems to increase exploration rate; however, communication considerations have been left largely unaddressed. This paper bridges this gap in the state of the art by developing distributed perceptual modeling that enables high-fidelity mapping while remaining amenable to low-bandwidth communication channels. The approach yields significant gains in exploration rate for multi-robot teams as compared to state-of-the-art approaches. The work is evaluated through simulation studies and hardware experiments in a wild cave in West Virginia.

==> content/abstract.tex <==
This work presents a framework for high-speed exploration of
extensive, cluttered environments with a multi-robot aerial system.
Robots are confined to separate regions of the environment and share
their environment models. The environment representation
leverages the compactness of approximate continuous belief
distributions for high-fidelity, real-time information sharing between
robots.  The approach demonstrates substantial gains in the rate of
information gain for the multi-robot exploration system as compared to
the single-robot exploration system in highly cluttered and unstructured
three-dimensional environments.

\keywords{robotic exploration, autonomous systems, motion planning, distributed mapping}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> content/experimental_insights.tex <==
\subsection{Experimental Insights\label{ssec:experimental_insights}}
Perceptual latency affects the maximum allowable speed during
exploration~\citep{goel2019fsr}. To leverage the compact perceptual
model for environment representation, software optimizations were
required to reduce the update time of the occupancy model. In addition, the
initialization strategy for the distributed mapping system works well
to produce a map of the environment using multiple robots, however the
global consistency can be improved using techniques from multi-robot
SLAM. During the experiment in the subterranean environment, the state
machine used for state transitions (\cref{ssec:implementation_detail})
was found to operate more reliably on a RF link compared to a WiFi
connection due to signal blockage from solid concrete located between the base station and the
robots.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> content/scheduled_experiments.tex <==
% commenting out because most of this is already stated in intro and results

% In this work, the problem of rapidly exploring aboveground and subterannean
% environments using a team of aerial robots is addressed by proposing a
% framework that enables high-speed exploration while using a compact
% representation of the environment to enable real-time distributed mapping.
% In aboveground operation, the robots were able to achieve maximum speeds in
% excess of $\SI{2.5}{m/s}$ while the communication requirements to transfer maps
% were found to be less than $8000$ bytes/s, suitable for low-bandwidth
% communication channels. Further experimentation is needed to test exploration
% in the subterranean environment, but other subsystems were tested.

Scheduled experiments will consist of extensive testing in a
variety of environments and conditions (e.g., larger distances between
robots). The performance will be evaluated by reporting the speeds
(see~\cref{sfig:speeds_scat} for example), data transferred
(see~\cref{sfig:comms_scat} for example), and system latency. Given
the current evolving conditions, we anticipate obtaining access to a
wider variety of test sites similar to~\textbf{E2} (i.e., subterranean
environments). In successive trials the communication bandwidth will
be progressively limited and data dropouts will be reported as a
function of communication bandwidth. Furthermore, the assumption of
multiple robots operating in disjoint spaces will be relaxed which
will require the implementation of a coordination strategy
to prevent collisions, aerodynamic interactions, and
violating the static world assumption for the state
estimator. Finally, a third robot will be introduced into the
multi-robot system and the effect of map sharing will be analyzed and reported.


==> preamble.tex <==
% to typeset URLs, URIs, and DOIs
\usepackage{url}
\def\UrlFont{\rmfamily}

% reduce figure caption size
\usepackage[font=footnotesize]{caption}

\usepackage[square,sort,comma,numbers]{natbib}

\usepackage{array}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{float}
\usepackage[capitalise]{cleveref}
\usepackage[binary-units=true]{siunitx}
\sisetup{per-mode=symbol,detect-weight=true}
\usepackage{subfig}
\usepackage{balance}

\usepackage{xcolor}
\usepackage{booktabs}

% Loads tikz plots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.16}

\usepackage{tikz}
% Load the library
\usetikzlibrary{external,positioning}
% Enable the library !!!>>> MUST be in the preamble <<<!!!!
\usepgfplotslibrary{external}
\tikzexternalize[prefix=tikzext/]

% Import Sarah Furnace Map
\usepackage{pdfpages}
\RequirePackage{luatex85}
\def\pgfsysdriver{pgfsys-pdftex.def}

% https://tex.stackexchange.com/questions/57484/is-there-a-way-to-control-whitespace-around-a-tikz-picture
\usepackage{adjustbox}

% To display all fbox'es around figures, set \vizfbox{true}
% To remove all fbox'es around figures set \vizfbox{false}
\newcommand\vizfbox{true}
\newcommand\vizbox[2]{\ifthenelse{\equal{#1}{false}}{\fbox{#2}}{#2}}

\definecolor{green}{RGB}{0,146,0}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{green}{#1}}}

